Active Inverse Learning in Stackelberg Trajectory Games

Game-theoretic inverse learning is the problem of inferring a player's objectives from their actions. We formulate an inverse learning problem in a Stackelberg game between a leader and a follower, where each player's action is the trajectory of a dynamical system. We propose an active inverse learning method for the leader to infer which hypothesis among a finite set of candidates best describes the follower's objective function. Instead of using passively observed trajectories like existing methods, we actively maximize the differences in the follower's trajectories under different hypotheses by optimizing the leader's control inputs. Compared with uniformly random inputs, the optimized inputs accelerate the convergence of the estimated probability of different hypotheses conditioned on the follower's trajectory. We demonstrate the proposed method in a receding-horizon repeated trajectory game and simulate the results using virtual TurtleBots in Gazebo.

==> numerical/numerical.tex <==
\section{Numerical Experiments}

We empirically demonstrate our results using a receding-horizon repeated trajectory game between a boundedly rational follower that controls one ground rover and a rational leader that controls multiple ground rovers. The leader is inferring which leading rover the follower is following. At each time step, the players play a Stackelberg trajectory game and implement only the first step of their respective input trajectories.    

We define the game parameters as follows. We model the dynamics of the following rover using an instance of \eqref{sys: leader lti}, where \(A^\fow = \exp\left(\delta\begin{bsmallmatrix}
    0_{2\times 2} & I_2\\
    0_{2\times 2} & 0_{2\times 2}
    \end{bsmallmatrix}\right)\), \(B^\fow=\int_{0}^\delta \exp\left(t\begin{bsmallmatrix}
    0_{2\times 2} & I_2\\
    0_{2\times 2} & 0_{2\times 2}
    \end{bsmallmatrix}\right)\mathrm{d}t \begin{bsmallmatrix}
    0_{2\times 2}\\
    I_2
    \end{bsmallmatrix}\), \(\Omega^\fow=\frac{1}{1000}I_4\), and \(\delta=0.2\) is the discretization step size. For the leader, we model the joint dynamics of \(d\in\mathbb{N}\) ground rovers using the joint dynamics of \(d\) double-integrators, where we let \(A^\lea = I_d\otimes A^\fow\), \(B^\lea =I_d\otimes B^\fow\), and \(\Omega^\lea=\frac{1}{1000}I_{4d\times 4d}\). For the follower's trajectory optimization in \eqref{opt: f-lqr}, we let \(Q^i = \diag(\begin{bsmallmatrix} 1 & 1& 0 & 0\end{bsmallmatrix} )\), \(R^i =\frac{1}{100}I_2\), and \(M^i = \begin{bsmallmatrix}
    0_{4\times 4(i-1)} & I_4 & 0_{4\times 4(d-i)}
    \end{bsmallmatrix}\) for all \(i\in[1, d]\). Without loss of generality, we assume \((Q^\fow, R^\fow, M^\fow, c^\fow)=(Q^1, R^1, M^1, c^i)\). For the leader's trajectory optimization in \eqref{opt: l-lqr}, we let \(\mathbb{U}\coloneqq\{u\in\mathbb{R}^{2d}|\norm{u}_\infty\leq 2\}\), and \(g(u^\lea_{0:\tau-1})=\sum_{t=1}^{\tau-2}\norm{u^\lea_{t+1}-u^\lea_t}^2\).

\begin{figure}[!ht]
\centering
     \subfloat[\(d=3\)\label{subfig: traj 3}]{%
     \centering
       \begin{tikzpicture}
    \begin{axis}[xlabel={\footnotesize horizontal position },
            ylabel={\footnotesize vertical position },
            xmin=-5, xmax=5,
            ymin=-5, ymax=5,
            width=0.5\columnwidth,
            height =0.5\columnwidth, 
            xtick={-4, 0, 4},
            xtick style={draw=none},
            ytick={-4, 0, 4},
            ytick style={draw=none},
            legend pos=south west,
             legend style={font=\footnotesize},
             yticklabel style = {font=\footnotesize},
            xticklabel style = {font=\footnotesize},
            ymajorgrids = true,
            xmajorgrids = true
    ]

 \addplot [mark=o, black, mark size=1pt] table [x=x1, y=y1, col sep=space]{numerical/3l_traj.dat};

 \addplot [mark=o, red,mark size=1pt] table [x=x2, y=y2, col sep=space]{numerical/3l_traj.dat};

 \addplot [mark=o, blue, mark size=1pt] table [x=x3, y=y3, col sep=space]{numerical/3l_traj.dat};

    \end{axis}  
    \end{tikzpicture}
     }
     \subfloat[\(d=5\)\label{subfig: traj 5}]{%
     \centering
        \begin{tikzpicture}
    \begin{axis}[
    xlabel={\footnotesize horizontal position },
            ylabel={\footnotesize vertical position },
    xmin=-5, xmax=5,
            ymin=-5, ymax=5,
            width=0.5\columnwidth,
            height =0.5\columnwidth, 
            xtick={-4, 0, 4},
            xtick style={draw=none},
            ytick={-4, 0, 4},
            ytick style={draw=none},
             legend pos=north east,
             legend style={font=\footnotesize},
             yticklabel style = {font=\footnotesize},
            xticklabel style = {font=\footnotesize},
            ymajorgrids = true,
            xmajorgrids = true
    ]

 \addplot [mark=o, orange, mark size=1pt] table [x=x1, y=y1, col sep=space]{numerical/5l_traj.dat};

 \addplot [mark=o, red, mark size=1pt] table [x=x2, y=y2, col sep=space]{numerical/5l_traj.dat};

 \addplot [mark=o, blue, mark size=1pt] table [x=x3, y=y3, col sep=space]{numerical/5l_traj.dat};

 \addplot [mark=o, teal, mark size=1pt] table [x=x4, y=y4, col sep=space]{numerical/5l_traj.dat};

 \addplot [mark=o, black, mark size=1pt] table [x=x5, y=y5, col sep=space]{numerical/5l_traj.dat};

    \end{axis}  
    \end{tikzpicture}
     }
     \caption{The position trajectories of the leader's rovers, where different rover's trajectories are marked by different colors.}
     \label{fig: traj}
\end{figure}

We demonstrate the proposed learning methods using the simulation of a receding-horizon repeated trajectory game. At time \(t\delta\) for some \(t\in\mathbb{N}\), the leader first observes its current state \(\overline{x}^\lea_t\) and the follower's current state \(\overline{x}^\fow_t\), then solves optimization~\eqref{opt: dcp} with \(\hat{x}_0^\lea=\overline{x}^\lea_t\) and \(\hat{x}^\fow_0=\overline{x}^\fow_t\) to obtain the optimal input sequence \(u^\lea_{0:\tau-1}\). Next, the leader simulates a state trajectory \(x^\lea_{0:\tau-1}\) according to \eqref{sys: leader lti} and shares it with the follower, then applies \(u^\lea_0\). Meanwhile, at time \(t\delta\), the follower observes its current state \(\hat{x}_t^\fow\) and receives the leader's simulated trajectory \(x_{0:\tau}^\lea\). Next the follower solves optimization~\eqref{opt: f-lqr} with \(\hat{x}^\fow_0=\overline{x}^\fow_t\) and obtain the optimal mean and covariance sequences \((\mu_{0:\tau-1}, \Sigma_{0:\tau-1})\), and finally samples \(u_0^\fow\sim\mathcal{N}(\mu_0, \Sigma_0)\) and applies \(u_0^\fow\) to its system. 

We simulate the players' trajectories in this receding-horizon repeated trajectory game by solving the leader's trajectory optimization~\eqref{opt: dcp} using the convex-concave procedure \cite{lipp2016variations}. Fig.~\ref{fig: traj} shows the position trajectories of the leader's rovers when \(d=3\) and \(d=5\). We can see that, to make the follower's trajectories under different hypotheses as different as possible, optimization~\eqref{opt: dcp} ensures that different leading rovers are moving in different directions. 

We further showcase the advantage of the proposed method in terms of distinguishing different hypotheses. To this end, we let \(p^\star= \begin{bmatrix}
    1 & 0 & \cdots & 0
\end{bmatrix}^\top\in\mathbb{R}^{d}\) denote the ground truth probability of all hypotheses (note that we let \((Q^\fow, R^\fow, M^\fow, c^\fow)=(Q^1, R^1, M^1, c^1)\)). In addition, we let \(p^t\) denote the \(d\)-dimensional vector such that
\begin{equation}
    p_i^t\coloneqq \mathds{P}((Q^\fow, R^\fow, M^\fow, c^\fow)= (Q^i, R^i, M^i, c^i)|\overline{x}^\fow_{0:t})
\end{equation}
for all \(i\in[1, d]\), where we let \(\mathds{P}((Q^\fow, R^\fow, M^\fow. c^\fow)= (Q^i, R^i, M^i, c^i)|\overline{x}^\fow_{0})\coloneqq \frac{1}{d}\) for all \(i\in[1, d]\), \ie, we choose the uniform distribution as the leader's prior distribution over all hypotheses given the follower's initial state. Notice that one can compute \(p^t\) recursively using the Bayes rule. Fig.~\ref{fig: Bayesian} shows the time history of the \(\ell_1\)-norm distance between \(p^t\) and \(p^\star\), and compare the results where the leader uses, instead of the inputs optimal for optimization~\eqref{opt: dcp}, independent and identically distributed input sampled from the uniform distribution over \(\mathbb{U}\). The results in Fig.~\ref{fig: Bayesian} show that, when compared with uniformly random inputs, the proposed method provide leader inputs that reduce the difference between \(p^t\) and \(p^\star\) by orders of magnitudes.    

\begin{figure}[!ht]
    \centering
    \begin{subfigure}[b]{\linewidth}
   \begin{tikzpicture}
    \begin{semilogyaxis}[
            xlabel={{\footnotesize Time steps \(t\)}},
            ylabel={{\footnotesize $\norm{p^t-p^\star}_1$}},
            xmin=0, xmax=10,
            ymin=1e-3, ymax=3,
            width=\columnwidth,
            height =0.5\columnwidth,
            xtick={0, 2, 4, 6, 8, 10},
            xtick pos=left,
            ytick={0.01, 0.1, 1},
            ytick style={draw=none},
           legend pos=south east,
             legend style={font=\footnotesize},
             yticklabel style = {font=\footnotesize},
            xticklabel style = {font=\footnotesize},
            ymajorgrids = true,
            xmajorgrids = true
    ]

     \addplot [yygreen, forget plot, mark=none, name path=p1, opacity=0.1] table [x=t, y=p1, col sep=space]{numerical/3l_belief.dat};
     \addplot [yygreen, forget plot, mark=none, , name path=p3, opacity=0.1] table [x=t, y=p3, col sep=space]{numerical/3l_belief.dat};
     \addplot[yygreen, forget plot, opacity=0.1] fill between[of=p1 and p3];
     
      \addplot [yygreen, thick, mark=none] table [x=t, y=p2, col sep=space]{numerical/3l_belief.dat};
      %\addlegendentry{Proposed Input}
      
         \addplot [yypurple, forget plot, mark=none, name path=q1, opacity=0.1] table [x=t, y=q1, col sep=space]{numerical/3l_belief.dat};
          \addplot [yypurple, forget plot, mark=none, name path=q3, opacity=0.1] table [x=t, y=q3, col sep=space]{numerical/3l_belief.dat};
           \addplot[yypurple, forget plot, opacity=0.1] fill between[of=q1 and q3];

      \addplot [yypurple, thick, mark=none] table [x=t, y=q2, col sep=space]{numerical/3l_belief.dat};
      %\addlegendentry{Random Input}
   
    \end{semilogyaxis}
    \end{tikzpicture}
     \caption{\(d=3\).}
    \end{subfigure}
\par\bigskip
\begin{subfigure}[b]{\linewidth}
   \begin{tikzpicture}
    \begin{semilogyaxis}[
            xlabel={{\footnotesize Time step \(t\)}},
            ylabel={{\footnotesize $\norm{p^t-p^\star}_1$}},
            xmin=0, xmax=10,
            ymin=1e-3, ymax=3,
            width=\columnwidth,
            height =0.5\columnwidth,
            xtick={0, 2, 4, 6, 8, 10},
            xtick pos=left,
            ytick={0.01, 0.1, 1},
            ytick style={draw=none},
            legend pos=south east,
             legend style={font=\footnotesize},
             yticklabel style = {font=\footnotesize},
            xticklabel style = {font=\footnotesize},
            ymajorgrids = true,
            xmajorgrids = true
    ]

    \addplot [yygreen, forget plot, mark=none, name path=p1, opacity=0.1] table [x=t, y=p1, col sep=space]{numerical/5l_belief.dat};
     \addplot [yygreen, forget plot, mark=none, , name path=p3, opacity=0.1] table [x=t, y=p3, col sep=space]{numerical/5l_belief.dat};
     \addplot[yygreen, forget plot, opacity=0.1] fill between[of=p1 and p3];
     
      \addplot [yygreen, thick, mark=none] table [x=t, y=p2, col sep=space]{numerical/5l_belief.dat};
      \addlegendentry{Proposed input}
      
         \addplot [yypurple, forget plot, mark=none, name path=q1, opacity=0.1] table [x=t, y=q1, col sep=space]{numerical/5l_belief.dat};
          \addplot [yypurple, forget plot, mark=none, name path=q3, opacity=0.1] table [x=t, y=q3, col sep=space]{numerical/5l_belief.dat};
           \addplot[yypurple, forget plot, opacity=0.1] fill between[of=q1 and q3];

      \addplot [yypurple, thick, mark=none] table [x=t, y=q2, col sep=space]{numerical/5l_belief.dat};
      \addlegendentry{Random input}
   
    \end{semilogyaxis}
    \end{tikzpicture}
     \caption{\(d=5\).}
    \end{subfigure}
    \caption{The comparison of the convergence of \(p^t\) when the leader obtains its input by solving optimization~\ref{opt: dcp} versus sampling uniformly in set \(\mathbb{U}\). The solid lines show the median over 100 simulations, while the boundaries of the colored areas mark the corresponding first and third quartiles.}
    \label{fig: Bayesian}
\end{figure}

==> related/related.tex <==
\section{Related Work}

{\bf Inverse learning in games} 

{\bf Active inverse reinforcement learning} 


